Deep Learning-based Denoising of Mammographic Images using Physics-driven Data Augmentation

Mammography is using low-energy X-rays to screen the human breast and is utilized by radiologists to detect breast cancer. Typically radiologists require a mammogram with impeccable image quality for an accurate diagnosis. In this study, we propose a deep learning method based on Convolutional Neural Networks (CNNs) for mammogram denoising to improve the image quality. We first enhance the noise level and employ Anscombe Transformation (AT) to transform Poisson noise to white Gaussian noise. With this data augmentation, a deep residual network is trained to learn the noise map of the noisy images. We show, that the proposed method can remove not only simulated but also real noise. Furthermore, we also compare our results with state-of-the-art denoising methods, such as BM3D and DNCNN. In an early investigation, we achieved qualitatively better mammogram denoising results.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% Horsch 041224
%
% - übernommen von Lehmann
% - angepasst für Proceedings BVM2003, Erlangen, Jan 2003
%	- Pseudo-Definitionen für tocgenerate (Generierung Inhaltsverz.)
%   \pagecount (Dez 2004)
%

\catcode`@=11

\def\makeauthor{\if@filesw \newwrite\@aindexfile
  \immediate\openout\@aindexfile=\jobname_authors.pix
  \def\addauthor{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wraindex}\typeout
  {Writing index file \jobname_authors.pix }\fi}

\def\@wraindex#1{
   \edef\@tempa{\write\@aindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addauthor{\@bsphack\begingroup \@sanitize\@addauthor}

\def\makepreindex{\if@filesw \newwrite\@pindexfile
  \immediate\openout\@pindexfile=\jobname_index.pix
  \def\addpreindex{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wrpindex}\typeout
  {Writing index file \jobname_authors.pix }\fi}

\def\@wrpindex#1{
   \edef\@tempa{\write\@pindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addpreindex{\@bsphack\begingroup \@sanitize\@addpreindex}

\def\makecategory{\if@filesw \newwrite\@bindexfile
  \immediate\openout\@bindexfile=\jobname_category.pix
  \def\addcategory{\@bsphack\begingroup
             \def\protect####1{\string####1\space}\@sanitize
             \@wrbindex}\typeout
  {Writing index file \jobname_category.pix }\fi}

\def\@wrbindex#1{
   \edef\@tempa{\write\@bindexfile{{#1}{\the\tocpos}}}
        \expandafter\endgroup\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

\def\addcategory{\@bsphack\begingroup \@sanitize\@addcategory}

\catcode`@=12




% \newcommand{\tocentry}[7]
\newcommand{\tocentry}[5]
% #1 = articletype + counter
% #2 = title
% #3 = Autoren
% #4 = Autoren, erster fett
% #5 = Seitenzahl
           {
            %\vspace{3mm}
            \noindent
%ho            \begin{minipage}[b]{115.5mm}
            \begin{minipage}[b]{114.5mm}
            \raggedright
            \begin{list}{}{\labelwidth9mm
                           \leftmargin9mm
                           \labelsep0mm}
%ho            \item[#1 \hfill] #3 \newline
%ho                        {\em #4}\dotfill
%             \item[#1 \hfill] {\em #2:} #4 #3 \dotfill
            \item[#1 \hfill] #3: #2 \dotfill  % #1 = Buchstabe und lfd. Nr.; #2 = Autoren; #3 = Autoren ;#4 = Titel
            \end{list}
            \end{minipage}
%ho            \begin{minipage}{5.5mm}
            \begin{minipage}{6.5mm}
%             \hfill\raisebox{1.5pt}{\the\tocpos} % Seitennummer
%             \hfill\raisebox{1.5pt} 
	      \hfill \raisebox{1.5pt}{#5}
            \end{minipage}
%             \addauthor{#5}
%             \addpreindex{#7}
%             \addcategory{#6}
%             \advance \tocpos #2\relax % advance erhöht/vermindert die Variable tocpos; relax macht nichts (no-op) = Abbruch ohne Fehlermeldung
%             \advance \tocpos \relax % advance erhöht/vermindert die Variable tocpos; relax macht nichts (no-op) = Abbruch ohne Fehlermeldung
        }


\newcommand{\firma}[1]
           {\begin{minipage}[t]{58mm}
             #1
            \end{minipage}}

\newcommand{\siehe}[2]{#2, {\it siehe} #1}

\newcommand{\nachsatz}[2]{#1, #2}

\newcommand{\nachsatzfett}[2]{#1, {\bf #2}}

\newcommand{\fett}[1]{{\bf #1}}

\newcommand{\fettumbruch}[1]{{\bf #1} \newpage}

\newcommand{\umbruch}[1]{#1 \newpage}

\newcommand{\zwischen}[1]
           {\newpage
            \rule{0mm}{0mm}

            \vspace{5cm}
            \begin{center}
            \baselineskip35pt
            {\huge \bf #1} 
            \end{center}}

%	Pseudo-Definition für tocgenerate
\newcommand{\pagecount}[1]{}


\newcommand{\elqq}{``}%
\newcommand{\erqq}{''}%
